Interactive Fiction Game Playing as Multi-Paragraph Reading Comprehension with Reinforcement Learning

Interactive Fiction (IF) games with real human-written natural language texts provide a new natural evaluation for language understanding techniques. In contrast to previous text games with mostly synthetic texts, IF games pose language understanding challenges on the human-written textual descriptions of diverse and sophisticated game worlds and language generation challenges on the action command generation from less restricted combinatorial space. We take a novel perspective of IF game solving and re-formulate it as Multi-Passage Reading Comprehension (MPRC) tasks. Our approaches utilize the context-query attention mechanisms and the structured prediction in MPRC to efficiently generate and evaluate action outputs and apply an object-centric historical observation retrieval strategy to mitigate the partial observability of the textual observations. Extensive experiments on the recent IF benchmark (Jericho) demonstrate clear advantages of our approaches achieving high winning rates and low data requirements compared to all previous approaches. Our source code is available at: https://github.com/XiaoxiaoGuo/rcdqn.

==> Text Games (camera-ready)/related_work.tex <==
\section{Related Work}

\paragraph{IF Game Agents.}
Previous work mainly studies the text understanding and generation in parser-based or rule-based text game tasks, such as TextWorld platform~\cite{cote2018textworld} or custom domains~\cite{narasimhan2015language,he2016deep,adhikari2020learning}. The recent platform \textit{Jericho}~\cite{hausknecht2019interactive} supports over thirty human-written IF games. 
Earlier successes in real IF games mainly rely on heuristics without learning. NAIL~\cite{hausknecht2019nail} is the state-of-the-art among these ``no-learning'' agents,  employing a series of reliable heuristics for exploring the game, interacting with objects, and building an internal representation of the game world.
With the development of learning environments like \textit{Jericho}, the RL-based agents have started to achieve dominating performance.

A critical challenge for learning-based agents is how to handle the \textbf{combinatorial action space} in IF games. LSTM-DQN~\cite{narasimhan2015language} was proposed to generate verb-object action with pre-defined sets of possible verbs and objects, but treat the selection and learning of verbs and objects independently. 
Template-DQN~\cite{hausknecht2019interactive} extended LSTM-DQN for template-based action generation, introducing one additional but still independent prediction output for the second object in the template.
Deep Reinforcement Relevance Network (DRRN)~\cite{he2016deep} was introduced for choice-based games.  Given a set of valid actions at every game state, DRRN projects each action into a hidden space that matches the current state representation vector for action selection. 
Action-Elimination Deep Q-Network (AE-DQN)~\cite{zahavy2018learn} learns to predict invalid actions in the adventure game \textit{Zork}. It eliminates invalid action for efficient policy learning via utilizing expert demonstration data.

% states 
Other techniques focus on addressing the \textbf{partial observability} in text games. 
Knowledge Graph DQN (KG-DQN)~\cite{ammanabrolu2019playing} was proposed to deal with synthetic games. The method constructs and represents the game states as knowledge graphs with objects as nodes and uses pre-trained general purposed OpenIE tool and human-written rules to extract relations between objects. KG-DQN handles the action representation following DRRN. 
KG-A2C~\cite{ammanabrolu2020graph} later extends the work for IF games, by adding information extraction heuristics to fit the complexity of the object relations in IF games and utilizing a GRU-based action generator to handle the action space.


\paragraph{Reading Comprehension Models for Question Answering.}
Given a question, reading comprehension (RC) aims to find the answer to the question based on a paragraph that may contain supporting evidence. One of the standard RC settings is extractive QA~\cite{rajpurkar2016squad,joshi2017triviaqa,kwiatkowski2019natural}, which extracts a span from the paragraph as an answer. 
Our formulation of IF game playing resembles this setting.

Many neural \emph{reader} models have been designed for RC. Specifically, for the extractive QA task, the reader models usually build question-aware passage representations via attention mechanisms~\cite{seo2016bidirectional,yu2018qanet}, and employ a pointer network to predict the start and end positions of the answer span~\cite{wang2016machine}.
% 
Powerful pre-trained language models~\cite{peters2018deep,devlin2019bert,radford2019language} have been recently applied to enhance the encoding and attention mechanisms of the aforementioned reader models. They give performance boost but are more resource-demanding and do not suit the IF game playing task very well.

\paragraph{Reading Comprehension over Multiple Paragraphs.}
Multi-paragraph reading comprehension (MPRC) deals with the more general task of answering a question from multiple related paragraphs, where each paragraph may not necessarily support the correct answer. Our formulation becomes an MPRC setting when we enhance the state representation with historical observations and predict actions from multiple observation paragraphs.

A fundamental research problem in MPRC, which is also critical to our formulation, is to select relevant paragraphs from all the input paragraphs for the reader to focus on.
Previous approaches mainly apply traditional IR approaches like BM25~\cite{chen2017reading,joshi2017triviaqa}, or neural ranking models trained with distant supervision~\cite{wang2018r,min2019discrete}, for paragraph selection. 
Our formulation also relates to the work of evidence aggregation in MPRC~\cite{wang2017evidence,lin2018denoising}, which aims to infer the answers based on the joint of evidence pieces from multiple paragraphs.
Finally, recently some works propose the entity-centric paragraph retrieval approaches~\cite{ding2019cognitive,godbole2019multi,min2019knowledge,asai2019learning}, where paragraphs are connected if they share the same-named entities. The paragraph retrieval then becomes a traversal over such graphs via entity links. These entity-centric paragraph retrieval approaches share a similar high-level idea to our object-based history retrieval approach.
The techniques above have been applied to deal with evidence from Wikipedia, news collections, and, recently, books~\cite{mou2020frustratingly}. We are the first to extend these ideas to IF games.



